Collision-Free Bearing-Driven Formation Tracking for Euler-Lagrange Systems

In this paper, we investigate the problem of tracking formations driven by bearings for heterogeneous Euler-Lagrange systems with parametric uncertainty in the presence of multiple moving leaders. To estimate the leaders' velocities and accelerations, we first design a distributed observer for the leader system, utilizing a bearing-based localization condition in place of the conventional connectivity assumption. This observer, coupled with an adaptive mechanism, enables the synthesis of a novel distributed control law that guides the formation towards the target formation, without requiring prior knowledge of the system parameters. Furthermore, we establish a sufficient condition, dependent on the initial formation configuration, that ensures collision avoidance throughout the formation evolution. The effectiveness of the proposed approach is demonstrated through a numerical example.

==> preamble.tex <==
\usepackage{indentfirst}
\usepackage{amsmath,amssymb}
\usepackage{graphicx,subfigure,epstopdf}
\usepackage{epic}
\usepackage{subfigure}
\usepackage{graphicx}
\usepackage{epsfig}
\usepackage{arydshln}
\usepackage{enumerate}
\usepackage[english]{babel}
\usepackage{fancyhdr}
\usepackage{lastpage}
\usepackage{color}
\usepackage{bm}
\usepackage{dsfont}
\usepackage{tikz}
\RequirePackage{spath3}
\usetikzlibrary{decorations.pathreplacing,calligraphy}
\usetikzlibrary{calc}
\usetikzlibrary{shadings}
\usepackage{caption}
\usepackage{changes}
\usepackage{pfdicons}
\usepackage{booktabs}
\usepackage{threeparttable}
\usepackage{animate}
\usepackage{natbib}
\usepackage{caption}
\usepackage[hyperfootnotes=false]{hyperref}
\usepackage{todonotes}
\hypersetup{
colorlinks=true,
linkcolor=black,
citecolor=cyan
}
\captionsetup{%
 % font=small,
  labelfont=bf,
  singlelinecheck=false,
  tableposition=top
}
\setcitestyle{longnamesfirst,round,authoryear,semicolon,sort&compress}

%\usepackage{mathbbold}
 \usepackage{amsmath}
\makeatletter
\def\underbracex#1#2{\mathop{\vtop{\m@th\ialign{##\crcr
   $\hfil\displaystyle{#2}\hfil$\crcr
   \noalign{\kern3\p@\nointerlineskip}%
   #1\crcr\noalign{\kern3\p@}}}}\limits}

\def\underbracea{\underbracex\upbracefilla}

\def\upbracefilla{$\m@th \setbox\z@\hbox{$\braceld$}%
  \bracelu\leaders\vrule \@height\ht\z@ \@depth\z@\hfill 
\kern\p@\vrule \@width\p@\kern\p@\vrule \@width\p@\kern\p@\vrule \@width\p@
$}

\def\underbraceb{\underbracex\upbracefillb}

\def\upbracefillb{$\m@th \setbox\z@\hbox{$\braceld$}%
\vrule \@width\p@\kern\p@\vrule \@width\p@\kern\p@\vrule \@width\p@\kern\p@
 \leaders\vrule \@height\ht\z@ \@depth\z@\hfill\bracerd
  \braceld\leaders\vrule \@height\ht\z@ \@depth\z@\hfill
\kern\p@\vrule \@width\p@\kern\p@\vrule \@width\p@\kern\p@\vrule \@width\p@
$}


\def\underbracec{\underbracex\upbracefillc}

\def\upbracefillc{$\m@th \setbox\z@\hbox{$\braceld$}%
\vrule \@width\p@\kern\p@\vrule \@width\p@\kern\p@\vrule \@width\p@\kern\p@
\leaders\vrule \@height\ht\z@ \@depth\z@\hfill
\kern\p@\vrule \@width\p@\kern\p@\vrule \@width\p@\kern\p@\vrule \@width\p@
$}

\def\underbraced{\underbracex\upbracefilld}
\def\upbracefilld{$\m@th \setbox\z@\hbox{$\braceld$}%
\vrule \@width\p@\kern\p@\vrule \@width\p@\kern\p@\vrule \@width\p@\kern\p@
 \leaders\vrule \@height\ht\z@ \@depth\z@\hfill\braceru$}

\def\underbracebd{\underbracex\upbracefillbd}
\def\upbracefillbd{$\m@th \setbox\z@\hbox{$\braceld$}%
\vrule \@width\p@\kern\p@\vrule \@width\p@\kern\p@\vrule \@width\p@\kern\p@
\bracerd\braceld
 \leaders\vrule \@height\ht\z@ \@depth\z@\hfill\braceru$}


\makeatother
\newcommand{\defeq}{\stackrel{\text{def}}{=}}
\newcommand{\myb}{\color{blue}}
\newcommand{\myr}{\color{red}}
%\setcitestyle{authoryear,colon}
%\usepackage[authoryear]{natbib}
%\usetikzlibrary{positioning}
%\newcounter{MYtempeqncnt}
%\newcommand{\defeq}{\stackrel{\text{def}}{=}}
\newcommand{\diag}{\mbox{diag}}
\newcommand{\col}{\mbox{col}}
%\renewcommand\thesection{\Roman{section}}
\newtheorem{Example}{Example}
\newtheorem{rem}{Remark}
\newtheorem{Corollary}{Corollary}
%\newtheorem{Definition}{Definition}
\newtheorem{Problem}{Problem}
\newtheorem{prop}{\it Property}
\newenvironment{proof}{\noindent{\em proof:\/}}{\hfill $\Box$\par}
\newtheorem{thm}{Theorem}
\newtheorem{lem}{Lemma}
\newtheorem{Conjecture}{Conjecture}
\newtheorem{ass}{Assumption}
\newtheorem{Property}{Property}
\newtheorem{proposi}{Proposition}
\newtheorem{Algorithm}{Algorithm}
\newcommand{\row}{\textnormal{row}}
\definecolor{mitRed}{RGB}{117,0,20}
\definecolor{mitSilverGray}{RGB}{139,149,158}
\definecolor{mitPurple}{RGB}{153,51,255}
\definecolor{mitBlue}{RGB}{25,102,255}
\definecolor{mitGreen}{RGB}{0,173,0}
\definecolor{mitLGreen}{RGB}{170,255,51}
\definecolor{mitPink}{RGB}{255,20,240}
\definecolor{mitLightPink}{RGB}{255,179,255}
\definecolor{mitDPink}{RGB}{117,0,98}
\definecolor{mitLightBlue}{RGB}{153,235,255}
\usetikzlibrary{shapes,arrows,positioning}
\newenvironment{Proof}{\noindent{\em Proof:\/}}{\hfill $\Box$\par}
%\newcommand{\tabref}[1]{Table~\ref{#1}}
\captionsetup[figure]{labelfont={bf},labelformat={default},labelsep=period,name={Fig.}}
\usetikzlibrary{decorations.markings}

\tikzset{test/.style n args={3}{
    postaction={
    decorate,
    decoration={
    markings,
    mark=between positions 0 and \pgfdecoratedpathlength step 0.5pt with {
    \pgfmathsetmacro\myval{multiply(
        divide(
        \pgfkeysvalueof{/pgf/decoration/mark info/distance from start}, \pgfdecoratedpathlength
        ),
        100
    )};
    \pgfsetfillcolor{#3!\myval!#2};
    \pgfpathcircle{\pgfpointorigin}{#1};
    \pgfusepath{fill};},
  mark=at position \pgfdecoratedpathlength with {\arrow[mitDPink,line width=#1] {>}; }
}}}}
